On monotone completion of risk markets: Limit results for incomplete risk markets

We consider a competitive market with risk-averse participants. We assume that agents' risks are measured by coherent risk measures introduced by Artzner et al. (1999). Fundamental theorems of welfare economics have long established the equivalence of competitive equilibria and system welfare optimization (see, e.g., Samuelson (1947)). These have been extended to the case of risk-averse agents with complete risk markets in Ralph and Smeers (2015). In this paper, we consider risk trading in incomplete markets and introduce a mechanism to complete the market iteratively while monotonically enhancing welfare.

==> figure_caption.tex <==
%Figure_1
\caption{\textbf{Improvement of social welfare through bundle refinement.} This figure illustrates the progression of incomplete markets towards the complete market social optimum and how refinement results in a non-decreasing trend.}

%Figure_2
\caption{Evolution of risk prices as bundles refine.}    
\caption{Bundle prices for two available trade bundles.}   %a
\caption{Bundle prices for four available trade bundles.}  %b
\caption{Bundle prices for eight available trade bundles.} %c

%Figure_3
\caption{Price progression of the bundle containing scenario 64 across refinement iterations}
\caption{Bundle prices at iteration $m = 4$.} %a
\caption{Bundle prices at iteration $m=5$.}   %b
\caption{Bundle prices at iteration $m=6$.}   %c
\caption{Bundle prices at iteration $m=7$.}   %d
\caption{Risk price in a complete market.}    %e

%Figure_4
\caption{Progression of risk price with bundle refinement.}
